To Intervene or Not: Guiding Inference-time Alignment with Probabilistic Model Blending

The wide deployment of LLMs has made model alignment necessary to make newly trained models safely and effectively respond to user instructions. Among different methods, inference-time alignment is often cheaper as it intervenes (i.e., offers guidances) only during output generation. Existing proposals apply guidances extracted from certain aligned models without properly assessing their reliability. Nonetheless, our systematic evaluation reveals that guidance effectiveness varies drastically across models; since ineffective guidances lead to further confusion and thus further interventions, the resulting excessive interventions typically indicate poor performance. To make interventions more effective and thus more efficient, we introduce BlendIn, an inference-time alignment framework that shifts from binary decisions to creating hybrid distributions integrating both models' knowledge. BlendIn stabilizes inference-time alignment by performing quality-aware alignment and proportionally weighting each model's contribution based on reliability. Compared with existing works, it preserves beneficial guidance while downweighting unreliable suggestions. BlendIn provides both diagnostic signals and mitigation strategies for misaligned guidance, achieving consistent and up to 50% performance improvement on challenging model pairs. Our code is available at: https://github.com/DecayingSeart/BlendIn.

==> cache/cache.tex <==


\begin{comment}
\begin{abstract}

\begin{comment}
%Despite the large success of LLM, 
As LLM gaining increasing
success,
% \revlx{popularization,}
requiring fine-tuning-based alignment with user instructions
%social norms to prevent harmful output 
for every newly trained model poses 
%a significant challenge for its 
%expensive
significant computational cost. 
\end{comment}

\revlx{As LLMs \revjg{get} widely deployed, performing fine-tuning–based alignment for every newly trained model 
to safely and effectively follow user instructions 
incurs substantial computational overhead.}
%cost is a problem
As a cheaper solution, 
inference-time alignment enables 
%pre-aligned 
aligned 
%small 
models to guide unaligned 
%large
models via intervening during output generation. 
%, offering an efficient alternative solution. 
% First say what is model family, why cross-fam is needed over within-fam
Existing 
%\revlx{plausible} 
works 
apply guidance 
%make aligned models intervene 
based on various signals extracted from aligned model. 
%whenever the unaligned model demonstrates high uncertainty.
However, they 
%focus on identifying when to intervene 
%but 
lack mechanisms to assess whether their guidance is truly reliable. %while   
%have achieved empirical success on specific 
%within-family 
%model pairs. %and
%. However, they 
%implicitly assuming that all guidance is beneficial.
%However, 
%they implicitly assume that all guidance is beneficial, while 
Our systematic evaluation reveals this oversight has severe consequences: guidance effectiveness varies dramatically across model pairs, with excessive interventions(>20\% of tokens generated) %frequently
systematically 
performing worse. %performance. %with %the opposite: 
%guidance quality varies significantly as 
%the importance of model compatibility and guidance quality, where
%higher intervention rates correlating with %\revjg{consistently} show 
%worse performance. 
%, where 
%weak guidance models over-intervene precisely because they provide low-quality suggestions.
%This paradox reveals 
This indicates that aligned %guidance 
models may also struggle %when unaligned model is uncertain, 
at the same positions where unaligned model have misaligned or harmful prediction, 
leading to misaligned generations and hence more interventions. 
%both intervene frequently due to their own uncertainty and 
%provide poor-quality suggestions. 
%, and naively aligning top tokens between models or capping intervention doesn't solve the problem.
%This indicates that 
%guidance quality varies dramatically, yet existing methods have no 
%diagnostic signals to predict or detect incompatibility.
%This reveals 
Such weakness reveals a quality blindness problem that treats harmful guidance and beneficial guidance identically, hindering greater success of inference time alignment in deployment. 
%This not only hinders greater empirical success but also provides %limited insight to future alignment designs on
%indicates the lack of
%mechanisms to assess model compatibility and guidance quality. %, 
%alignment performance under cross-family scenarios remains underwhelming, largely due to a lack of principled understanding that predicts cross-family model compatibility, 
%add they lack principled understanding?
%, despite empirical successes ~\cite{},
%a deep understanding of the conditions under which smaller models succeed or fail in aligning bigger models remains limited, 
%hindering greater empirical successes and providing limited insights to future method designs.
%a deep understanding of when and why a smaller model may align a larger model remains limited. 
%their effectiveness across capability gaps remains unvalidated
%To fill this gap, we conducted the first systematic analysis of cross-family inference-time alignment 
%of inference-time alignment 
%across nine models and six benchmarks, uncovering
%an %intervention paradox where 
%model pairs with 
%principles where 
%Our systematic evaluation reveals that this assumption fails: higher intervention rates consistently show worse performance and 
%(r=-0.65 to -0.76, p<0.03).
%Despite the challenge of identifying the cause of this correlation, through comprehensive 
%vocabulary analysis and
%cross-family 
%experiments, we demonstrate that this paradox reflects 
%the importance of 
%guidance quality matters more than quantity.
%, as weak models intervene more frequently and provide poorer guidance. 
%Based on these insights, 
\begin{comment}
To address this gap, we introduce \name, 
%an distribution-blending method that 
%selectively accepts guidance aligned with the base model's preferences
which 
adaptively blends probability distributions from both models 
to sample tokens proportionally to their \newrev{guidance} quality, 
%for a comprehensive decision,
achieving \needrev{maximum 50\%} improvement on challenging %high-intervention
%cross-family 
model pairs. %while enabling rapid model compatibility diagnosis. 
Our work provides the first systematic analysis of quality failures in inference-time alignment, 
%when and why inference-time alignment fails, 
establishing both diagnostic signal and effective mitigation strategy for practical deployment.
%insights for deploying inference-time alignment% and reveal fundamental insights about model compatibility.
\end{comment}
\revlx{To address this gap, we introduce \name, an inference-time alignment framework that weights guidance based on respective certainties of aligned and unaligned models. 
%adaptively integrates probability distributions from \revjg{both aligned and unaligned} models to sample tokens in proportion to their \newrev{token} quality.
\name provides both diagnostic signals and mitigation strategies for %real-world deployment,
misaligned or harmful guidance, achieving consistent and up to \revjg{50\%} performance improvement on challenging model pairs.}
%effective mitigation strategies

\end{abstract}
\end{comment}
